Efficient Algorithms for Densest Subgraph Discovery

Densest subgraph discovery (DSD) is a fundamental problem in graph mining. It has been studied for decades, and is widely used in various areas, including network science, biological analysis, and graph databases. Given a graph G, DSD aims to find a subgraph D of G with the highest density (e.g., the number of edges over the number of vertices in D). Because DSD is difficult to solve, we propose a new solution paradigm in this paper. Our main observation is that a densest subgraph can be accurately found through a k-core (a kind of dense subgraph of G), with theoretical guarantees. Based on this intuition, we develop efficient exact and approximation solutions for DSD. Moreover, our solutions are able to find the densest subgraphs for a wide range of graph density definitions, including clique-based and general pattern-based density. We have performed extensive experimental evaluation on eleven real datasets. Our results show that our algorithms are up to four orders of magnitude faster than existing approaches.

==> pdsCore.tex <==
\subsection{Optimization for Core Decomposition}

The core decomposition algorithm in Section~\ref{sec:decompose} can be extended for a general pattern $\Psi$. For particular patterns, such as stars, and loops, the decomposition process above can be performed faster, because the two key steps -- \emph{computing the pattern-degrees} and \emph{decreasing the vertices' pattern-degrees}, can be done more efficiently.
In the following, we illustrate this for two kinds of commonly encountered patterns, namely \emph{star}, and \emph{loop}.

\noindent \textbf{1 Star Patterns.}
The star pattern has been widely investigated~\cite{nature2003,leskovec2006,nature2010}. Specifically, a star pattern consists of a star-vertex (center) with a few tail-vertices (spokes). We call a star pattern with $x$ ($x\textgreater$1) tail-vertices an $x$-star pattern. In Figure~\ref{fig:starGraph}(a), we depict the 3-star pattern $\Psi$. The whole graph in Figure~\ref{fig:starGraph}(b) is an example (3, $\Psi$)-core: each vertex participates in at least three 3-star pattern instances.

\begin{figure}[h]
\hspace*{-.1cm}
\centering
\begin{tabular}{c c c}
  \begin{minipage}{2.2cm}
	\includegraphics[width=2.2cm]{figures/star-motif}
  \end{minipage}
  &
  \begin{minipage}{1.40cm}
	\includegraphics[width=1.40cm]{figures/star-core}
  \end{minipage}
  &
  \begin{minipage}{1.40cm}
	\includegraphics[width=1.40cm]{figures/diamond}
  \end{minipage}
  \\
  (a) 3-star
  &
  (b) (3, $\Psi$)-core ($\Psi$=3-star)
  &
  (c) diamond
\end{tabular}
\caption{Illustrating the special patterns.}
\label{fig:starGraph}
\end{figure}

Given an $x$-star pattern, we now discuss how to efficiently perform these two key steps for a vertex $v$ during the decomposition process. Assume that $v$ has $y$ neighbors, and let $v$'s $i$-th (1$\leq i\leq y$) neighbor be $u$.

\textbf{\underline{1.1 Computing $v$'s pattern-degree.}}
There are two disjoint cases: (1) $v$ is the star-vertex and (2) $v$ is a tail-vertex.
For case (1), the number of pattern instances is ${y \choose x}$,
since any $x$ neighbors of $v$ can form a $x$-star with $v$.
For case (2), the number of pattern instances is
$\sum\limits_{1 \le i \le y \wedge x \le z_i} {{z_i-1} \choose x-1}$,
where $z_i$ is $u$'s degree, since $v$ and any other $x$--1 neighbors of $u$ can form a $x$-star with $u$.
Therefore, we have
\begin{equation}
\small
deg_G(v, \Psi)={y \choose x} + \sum\limits_{1 \le i \le y \wedge x \le z_i} {{{z_i-1} \choose x-1}}.
\end{equation}
Here, we adopt the convention that ${y \choose x} =0$, whenever $y\textless x$.

%\note[Laks]{What if the $i$-th neighbor of $v$ has degree $z_i < x$? Similarly, what if $y < x$? We should mention in those cases, the term is assumed to be $0$ w.l.o.g.}

\textbf{\underline{1.2 Decreasing pattern-degrees.}}
After removing $v$, we also have two disjoint cases:
(1) decreasing the pattern-degrees of $v$'s 1-hop neighbors,
and (2) decreasing the pattern-degrees of $v$'s 2-hop neighbors.
Let us denote $v$'s $i$-th (1$\leq i\leq y$) neighbor by $u$.
For case (1), we have to compute the number of pattern instances that include both $v$ and $u$.
When $v$ is the star-vertex, the number of $x$-stars that have a tail-vertex $u$ is ${{y-1} \choose {x-1}}$,
since $u$ and any other $x$--1 neighbors of $v$ can form a $x$-star with $v$;
when $v$ is the tail-vertex, the number of $x$-stars that have a star-vertex $u$ is ${{z_i-1} \choose {x-1}}$,
since $v$ and any other $x$--1 neighbors of $u$ can form a $x$-star with $u$.
Therefore, we decrease $u$'s pattern-degree by
${{y-1} \choose {x-1}}+{{z_i-1} \choose {x-1}}$.

%\note[Laks]{What is the rationale for the first term?}

In case (2), $u$ must be a star-vertex and $v$ is a tail-vertex. For each neighbor $w$ of $u$ ($w\neq v$), we need to decrease $w$'s pattern-degree by ${{z_i-2} \choose {x-2}}$, because $v$, $w$, and any other $x$--2 neighbors of $u$ can form an $x$-star with $u$.
%\note[Laks]{Again, you should explain the rationale.}

From the discussions above, we can easily conclude that, the first and second steps can be completed in ${\mathcal O}(d)$ and ${\mathcal O}(d^2)$ time respectively, because we only need to enumerate their 1-hop and 2-hop neighbors. Note that the values of different ${y \choose x}$ ($x$$\leq$$y$$\leq$$d$) can be precomputed in advance. Therefore, for any $x$-star pattern, the time cost of performing $k$-pattern-core decomposition can be reduced from ${\mathcal O}\left( {n \cdot d^x} \right)$ to ${\mathcal O}(n\cdot{d^2})$.

\noindent \textbf{2 Loop Patterns.}
For ease of exposition, we take the diamond pattern (see Figure~\ref{fig:starGraph}(c)) as an example to illustrate the details of these two steps. The diamond pattern has also been used in many real applications~\cite{nature2003,leskovec2006,diamond2014}.
%We now discuss how to perform the two steps efficiently, w.r.t.the diamond pattern.

%\noindent
\textbf{\underline{2.1 Computing $v$'s pattern-degree.}}
We first enumerate all the paths from $v$ to its 2-hop neighbors, and then organize these paths into $h$ groups, each of which share the same 2-hop neighbor. Then, for each group, any pair of paths can form an instance of the diamond pattern.
Let the size of the $i$-th group be $y_i$ ($1\leq i\leq h$). We thus have $de{g_G}(v,\Psi) = \sum\limits_{1 \le i \le h \wedge {y_i} \ge 2} {y_i \choose 2}$.

%\noindent
\textbf{\underline{2.2 Decreasing pattern-degrees.}}
We handle the groups one by one. Consider the specific group $h_i$, which only has one 2-hop neighbor of $v$.
If $y_i$=1, we skip this group as there is not any pattern instance.
If $y_i\geq 2$, we decrease the pattern-degree of the 2-hop neighbor by ${y_i \choose 2}$.
%
%\note[Laks]{This doesn't seem right. $de{g_G}(v,\Psi)$ is the total contribution to $v$'s pattern degree from all the groups and it should not be subtracted from the curent pattern degree of a specific 2-hop neighbor of $v$. It seems we should just subtract $y_i\choose 2$.}
%
For each 1-hop neighbor in $g_i$, we decrease its pattern-degree by $y_i$--1, because each path participates in $y_i$--1 pattern instances.

Clearly, the time complexity of performing the two steps above is ${\mathcal O}(d^2)$. Hence,
the time cost of performing core decomposition is reduced from ${\mathcal O}\left( {n \cdot d^3} \right)$ to ${\mathcal O}(n\cdot{d^2})$.

\noindent\textbf{Remark.} For other general patterns, if more efficient pattern enumeration algorithms are known or devised in the future, the efficiency of their core decomposition can be improved.


==> proof-sec6.1.tex <==
\subsection{Proofs for Section~\ref{sec:advancedExact}}
\label{sec:proofAdvancedExact}

\noindent\textbf{Lemma}~\ref{lemma:prunePattern}.
\emph{Given a graph $G$ and an $h$-clique $\Psi$, for any clique instance $\psi$, let $G'$ be the residual subgraph of $G$ after removing all the vertices of $\psi$ from $G$. If we have $\rho (G', \Psi) > \rho (G, \Psi)$, then we do not need to create a node for $\psi$ in the flow network.}

\begin{proof}
For any clique instance $\psi\in G$ pruned by Lemma~\ref{lemma:prunePattern}, let $X$ be the set of its vertices, and $D(V_D, E_D)$ be the CDS of $G$. We firstly prove that $|X\bigcap (V\backslash V_D)|\geq 1$, which means that at least one vertex of $\psi$ is not in the CDS.
According to Lemma~\ref{lemma:prune}, we can easily prove it by contradiction. Assume that $X\subseteq V_D$, then
\begin{equation}
\begin{array}{l}
\rho (G\backslash \psi ,\Psi ) \le \frac{{\rho (G,\Psi )|V| - \rho (D,\Psi )|{V_\psi }|}}{{|V| - |{V_\psi }|}}\\
 \le \frac{{\rho (G,\Psi )(|V| - |{V_\psi }|)}}{{|V| - |{V_\psi }|}} = \rho (G,\Psi ).
\end{array}
\end{equation}
However, this contradicts our assumption above. Hence, we conclude that at least one vertex of $\psi$ is not in the CDS.

Next, we prove that after removing $\psi$ from the flow network ${\mathcal F}$, we can compute the CDS correctly by using the flow network. Since our algorithm follows the same framework with the exact algorithm in \cite{tsourakakis2015k}. According to \cite{tsourakakis2015k}, to prove the correctness of the exact CDS algorithm, we need to prove the following two cases:

\begin{enumerate}
  \item if there is a subgraph with vertex set $Y$ s.t. $\rho(G[Y], \Psi)\textgreater\alpha$, then any minimum st-cut ($\mathcal S$, $\mathcal T$) of ${\mathcal F}$ has $\mathcal S\backslash$\{$s$\}$\ne\emptyset$;
  \item if there does not exist a subgraph with vertex set $Y$ such that $\rho(G[Y], \Psi)\textgreater\alpha$, then the minimum st-cut satisfies that $\mathcal S$=\{$s$\} and $\mathcal T$=$\mathcal A\cup\mathcal B\cup$\{$t$\}.
\end{enumerate}

For ease of presentation, we introduce a notation, $\Psi [R, i]$, to indicate the number of clique instances that involve exactly $i$ ($1\leq i\leq |V_\Psi|$) vertices from a given set $R$ of vertices. According to \cite{tsourakakis2015k}, given a flow network ${\mathcal F}(V_{\mathcal F}, E_{\mathcal F})$ constructed by Algorithm in \cite{tsourakakis2015k}, let (${\mathcal S}$, ${\mathcal T}$) denote its minimum st-cut,
${\mathcal A_1}$=${\mathcal S}\bigcap {\mathcal A}$,
${\mathcal B_1}$=${\mathcal S}\bigcap {\mathcal B}$,
${\mathcal A_2}$=${\mathcal T}\bigcap {\mathcal A}$, and
${\mathcal B_2}$=${\mathcal T}\bigcap {\mathcal B}$.
Then, the capacity of the minimum st-cut is
$\Phi  + \alpha \cdot|{V_\Psi }|\cdot|{\mathcal{A}_1}| + \Pi$,
where $\Phi$=$\sum\limits_{v \notin {\mathcal A_1}} {de{g_G}} (v,\Psi )$, and $\Pi=\sum\limits_{i = 1}^{|{V_\Psi }| - 1} i \cdot\Psi [{\mathcal A_1},i]$.

Notice that the flow network constructed by {\tt CoreExact} has the same structure and capacity with the one in \cite{tsourakakis2015k}, so after removing $\psi$ from $\mathcal F$, we need to decrease the clique-degree of each vertex of $\psi$ by one. Then, the capacity of the minimum st-cut is
\begin{equation}
\label{eq:pruneCliqueNewVLDB}
\Phi'+\alpha \cdot|{V_\Psi }|\cdot|{\mathcal A_1}|+\Pi',
\end{equation}
where $\Phi'$=$\sum\limits_{v \notin {\mathcal A_1}} {de{g_G}} (v,\Psi )$--1, and $\Pi'$=$\sum\limits_{i = 1}^{|{V_\Psi }| - 1} i \cdot\Psi[{\mathcal A_1},i]'$ (Here, $\Psi[{\mathcal A_1},i]'$ is the number of clique instance that involve exactly $i$ vertices from the vertex set $\mathcal A_1$, after removing $\psi$).

Next, we prove that the two cases above still hold.

\noindent\textbf{\underline{First case:}}
We prove it by contradiction. Suppose that there is a subgraph with vertex set $Y$ such that $\rho(G[Y], \Psi)\textgreater\alpha$ and the minimum st-cut is achieved by $(\{s\},\mathcal A\cup \mathcal B\cup \{t\})$. In this case the capacity of the minimum st-cut is
\begin{equation}
\label{eq:firstTermVLDB}
\sum_{v\in \mathcal A} deg_G(v, \Psi)=|V_\Psi|\mu(G,\Psi).
\end{equation}

We now consider another different st-cut ($\mathcal S$, $\mathcal T$), where $\mathcal S$=\{$s$\}$\cup\mathcal A_1\cup\mathcal B_1$, $\mathcal A_1$=$Y$, $\mathcal B_1$ is the set of groups of pattern instances formed by vertices in $\mathcal A_1$, and $\mathcal T$ contains the rest nodes in the network $\mathcal F$. Then, the capacity of this st-cut is exactly Eq~(\ref{eq:pruneCliqueNewVLDB}).

Since we assume that the minimum st-cut is achieved by $(\{s\},\mathcal A\cup \mathcal B\cup \{t\})$, the relationship between Eqs~(\ref{eq:pruneCliqueNewVLDB}) and (\ref{eq:firstTermVLDB}) can be represented as
\begin{equation}
\label{eq:compareVLDB}
\footnotesize
\sum\limits_{v \in {\mathcal A}} d e{g_G}(v,\Psi ) \le
\Phi'+\alpha \cdot|{V_\Psi }|\cdot|{\mathcal A_1}|+\Pi',
%\sum\limits_{v \notin {{\mathcal A}_1}} d e{g_G}(v,\Psi ) + \alpha  \cdot |{V_\Psi }| \cdot |{{\mathcal A}_1}| + \sum\limits_{i = 1}^{|{V_\Psi }| - 1} i  \cdot \Psi [{{\mathcal A}_1},i].
\end{equation}

Then, the left part is
\begin{equation}
\sum\limits_{v \in {\mathcal A}} d e{g_G}(v,\Psi )=\Phi'+|{V_\Psi }|\cdot\Psi [{{\mathcal A}_1},|{V_\Psi }|]+\Pi'.
\end{equation}

Therefore, the Eq~(\ref{eq:compareVLDB}) can be represented as
\begin{equation}
\Phi'+|{V_\Psi }|\cdot\Psi [{{\mathcal A}_1},|{V_\Psi }|]+\Pi'\leq \Phi'+\alpha \cdot|{V_\Psi }|\cdot|{\mathcal A_1}|+\Pi'.
\end{equation}
We can further simply the inequation above as
\begin{equation}
|{V_\Psi }| \cdot \Psi [{{\mathcal A}_1},|{V_\Psi }|] \le \alpha  \cdot |{V_\Psi }| \cdot |{{\mathcal A}_1}|.
\end{equation}

Since $|V_\Psi|\geq 1$, $|{V_\Psi }| \cdot \Psi [{{\mathcal A}_1}, |{V_\Psi }|]$=$\mu(G[Y], \Psi)$, and $|\mathcal A_1|$=$|Y|$, we can conclude that $\rho (G[Y],\Psi ) = \frac{{\mu (G[Y],\Psi )}}{{|Y|}} \le \alpha$,
which contradicts the assumption. Hence the first case holds.

\noindent\textbf{\underline{Second case:}}
Similar to the the proof of first case, we can also prove that the second case also holds by contradiction.

Hence, after removing $\psi$ from flow network, we can still find the CDS by computing the minimum st-cut, although the value of minimum st-cut may be different.
\end{proof}

